SAILOR: Scaling Anchors via Insights into Latent Object Representation

LiDAR 3D object detection models are inevitably biased towards their training dataset. The detector clearly exhibits this bias when employed on a target dataset, particularly towards object sizes. However, object sizes vary heavily between domains due to, for instance, different labeling policies or geographical locations. State-of-the-art unsupervised domain adaptation approaches outsource methods to overcome the object size bias. Mainstream size adaptation approaches exploit target domain statistics, contradicting the original unsupervised assumption. Our novel unsupervised anchor calibration method addresses this limitation. Given a model trained on the source data, we estimate the optimal target anchors in a completely unsupervised manner. The main idea stems from an intuitive observation: by varying the anchor sizes for the target domain, we inevitably introduce noise or even remove valuable object cues. The latent object representation, perturbed by the anchor size, is closest to the learned source features only under the optimal target anchors. We leverage this observation for anchor size optimization. Our experimental results show that, without any retraining, we achieve competitive results even compared to state-of-the-art weakly-supervised size adaptation approaches. In addition, our anchor calibration can be combined with such existing methods, making them completely unsupervised.

==> table_to_kitti_extensive.tex <==
\begin{table*}
  \begin{center}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{c c c c c c c c c c c}
        \toprule[1pt]
             &            & \multicolumn{3}{c}{Car}        & \multicolumn{3}{c}{Pedestrian}              & \multicolumn{3}{c}{Cyclist}                                                                                                                                                                                                                                                                                                     \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        Task & Method     & Easy                           & Moderate                                    & Hard                                        & Easy                                        & Moderate                                    & Hard                                        & Easy                                        & Moderate                                    & Hard                                        \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
        \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11}
        \multirowcell{6}{Waymo                                                                                                                                                                                                                                                                                                                                                                                                             \\ $\downarrow$ \\ KITTI} & SA     & $74.36$ / $24.46$       & $64.97$ / $23.93$ & $63.09$ / $21.77$ & $68.87$ / $65.18$ & $64.00$ / $59.98$ & $59.77$ / $56.21$ & $61.27$ / $58.82$ & $54.29$ / $52.32$ & $52.03$ / $49.80$  \\
        \cmidrule(lr){2-11}
             & SN$^\dag$  & $80.91$ / $27.03$              & $68.77$ / $24.11$                           & $66.06$ / $22.44$                           & $\bestresult{70.38}$ / $\bestresult{69.22}$ & $\bestresult{66.10}$ / $\bestresult{63.51}$ & $\bestresult{64.68}$ / $\bestresult{59.41}$ & $64.06$ / $60.54$                           & $54.63$ / $52.83$                           & $52.65$ / $50.97$                           \\
             & OT$^\dag$  & $72.25$ / $43.26$              & $67.07$ / $38.79$                           & $67.69$ / $39.43$                           & $62.99$ / $57.77$                           & $58.52$ / $53.31$                           & $55.62$ / $49.69$                           & $\bestresult{73.38}$ / $\bestresult{72.08}$ & $\bestresult{63.14}$ / $\bestresult{61.82}$ & $\bestresult{60.65}$ / $\bestresult{57.27}$ \\
             & ROS$^\dag$ & $\bestresult{83.41}$ / $45.94$ & $74.57$ / $43.00$                           & $74.71$ / $41.76$                           & $68.88$ / $66.52$                           & $63.01$ / $62.39$                           & $59.59$ / $57.84$                           & $59.70$ / $57.17$                           & $51.85$ / $51.09$                           & $49.22$ / $48.49$                           \\
             & TA$^\dag$  & $55.92$ / $38.50$              & $60.96$ / $39.69$                           & $66.43$ / $45.17$                           & $58.51$ / $54.08$                           & $54.07$ / $49.95$                           & $51.51$ / $47.16$                           & $68.34$ / $64.00$                           & $58.67$ / $55.45$                           & $55.34$ / $52.58$                           \\
        \cmidrule(lr){2-11}
             & Ours       & $82.53$ / $\bestresult{61.10}$ & $\bestresult{79.90}$ / $\bestresult{58.02}$ & $\bestresult{80.13}$ / $\bestresult{58.88}$ & $69.63$ / $67.66$                           & $63.86$ / $61.60$                           & $60.58$ / $57.47$                           & $64.47$ / $60.35$                           & $56.78$ / $53.04$                           & $54.18$ / $50.90$                           \\
        \midrule
        \multirowcell{6}{nuScenes                                                                                                                                                                                                                                                                                                                                                                                                          \\ $\downarrow$ \\ KITTI} & SA & $83.00$ / $34.21$ & $68.48$ / $26.37$ & $67.30$ / $25.38$ & $16.62$ / $11.95$ & $14.90$ / $10.37$ & $12.60$ / $\phantom{0}9.43$ & $37.80$ / $31.68$ & $27.97$ / $22.90$ & $26.80$ / $22.00$ \\
        \cmidrule(lr){2-11}
             & SN$^\dag$  & $72.09$ / $40.74$              & $59.18$ / $33.67$                           & $58.59$ / $30.70$                           & $\bestresult{37.79}$ / $\bestresult{34.12}$ & $\bestresult{34.92}$ / $\bestresult{31.67}$ & $\bestresult{32.53}$ / $\bestresult{29.80}$ & $26.68$ / $15.31$                           & $25.37$ / $14.29$                           & $24.36$ / $10.41$                           \\
             & OT$^\dag$  & $83.54$ / $48.02$              & $72.29$ / $36.42$                           & $69.32$ / $35.00$                           & $22.51$ / $19.34$                           & $20.71$ / $18.15$                           & $19.90$ / $17.40$                           & $28.58$ / $12.43$                           & $24.04$ / $\phantom{0}8.84$                 & $23.54$ / $\phantom{0}8.74$                 \\
             & ROS$^\dag$ & $\bestresult{89.42}$ / $73.34$ & $\bestresult{75.97}$ / $56.28$              & $\bestresult{74.74}$ / $54.93$              & $32.46$ / $29.95$                           & $29.41$ / $26.88$                           & $27.54$ / $24.06$                           & $26.08$ / $25.11$                           & $20.23$ / $19.76$                           & $19.42$ / $18.35$                           \\
             & TA$^\dag$  & $82.98$ / $\bestresult{68.29}$ & $72.87$ / $\bestresult{57.93}$              & $72.11$ / $\bestresult{56.48}$              & $22.68$ / $19.71$                           & $21.00$ / $18.57$                           & $19.99$ / $17.55$                           & $24.71$ / $14.35$                           & $20.72$ / $11.67$                           & $20.33$ / $11.48$                           \\
        \cmidrule(lr){2-11}
             & Ours       & $83.71$ / $67.72$              & $72.76$ / $55.10$                           & $71.31$ / $53.52$                           & $\phantom{0}5.56$ / $\phantom{0}4.64$       & $\phantom{0}5.53$ / $\phantom{0}4.64$       & $\phantom{0}5.40$ / $\phantom{0}4.65$       & $\bestresult{38.83}$ / $\bestresult{35.31}$ & $\bestresult{29.88}$ / $\bestresult{26.37}$ & $\bestresult{28.50}$ / $\bestresult{25.02}$ \\
        \midrule
        \multirowcell{6}{Lyft \\ $\downarrow$ \\ KITTI} & SA & $\bestresult{89.10}$ / $74.06$ & $78.25$ / $62.22$ & $77.20$ / $56.44$ & $55.55$ / $52.86$ & $48.45$ / $46.97$ & $\bestresult{46.30}$ / $42.74$ & $60.74$ / $59.20$ & $53.74$ / $\bestresult{51.54}$ & $50.72$ / $\bestresult{49.00}$  \\
        \cmidrule(lr){2-11}
             & SN$^\dag$  & $88.25$ / $69.56$              & $77.17$ / $54.90$                           & $75.33$ / $52.47$                           & $\bestresult{56.21}$ / $\bestresult{53.59}$                           & $\bestresult{48.61}$ / $\bestresult{47.32}$                           & $46.28$ / $\bestresult{44.34}$                           & $61.41$ / $\bestresult{59.22}$                           & $52.92$ / $51.48$                           & $51.11$ / $\bestresult{49.00}$                           \\
             & OT$^\dag$  & $71.26$ / $29.77$              & $67.93$ / $28.46$                           & $68.53$ / $31.61$                           & $51.15$ / $46.36$                           & $46.80$ / $41.06$                           & $42.47$ / $38.84$                           & $\bestresult{62.36}$ / $49.50$                           & $\bestresult{54.70}$ / $39.78$                           & $\bestresult{51.89}$ / $38.09$                           \\
             & ROS$^\dag$ & $86.02$ / $62.77$              & $72.47$ / $48.95$                           & $67.11$ / $43.79$                           & $54.92$ / $52.50$                           & $48.38$ / $46.44$                           & $45.27$ / $42.15$                           & $62.13$ / $58.74$                           & $53.12$ / $49.98$                           & $49.64$ / $46.48$                           \\
             & TA$^\dag$  & $84.11$ / $63.62$              & $74.95$ / $54.85$                           & $75.26$ / $55.99$                           & $50.82$ / $45.22$                           & $45.42$ / $40.03$                           & $40.89$ / $37.51$                           & $58.90$ / $48.48$                           & $51.11$ / $37.77$                           & $48.46$ / $35.54$                           \\
        \cmidrule(lr){2-11}
             & Ours       & $88.55$ / $\bestresult{83.87}$              & $\bestresult{84.00}$ / $\bestresult{73.85}$                           & $\bestresult{82.05}$ / $\bestresult{71.06}$                           & $50.04$ / $45.12$                           & $46.06$ / $46.06$                           & $42.60$ / $40.36$                           & $58.82$ / $54.03$                           & $50.40$ / $44.21$                           & $48.72$ / $41.73$                           \\
        \bottomrule[1pt]
      \end{tabular}
    }
  \end{center}
  \caption{
    Results of the adaptation from Waymo, nuScenes and Lyft to KITTI, for different classes and difficulties.
    We report AP$_{BEV}$ / AP$_{3D}$.
    We compare our method to Source Anchors (SA), Statistical Normalization (SN), Output Transformation (OT), Random Object Scaling (ROS) and Target Anchors (TA).
    $^\dag$ denotes weakly-supervised methods.
  }
  \label{table:to_kitti_extnsive}
\end{table*}


==> table_to_waymo_extensive.tex <==
\begin{table*}
  \begin{center}
    \resizebox{\linewidth}{!}{
      \begin{tabular}{c c c c c c c c c c c}
        \toprule[1pt]
             &            & \multicolumn{3}{c}{Vehicle}                 & \multicolumn{3}{c}{Pedestrian}                            & \multicolumn{3}{c}{Cyclist}                                                                                                                                                                                                                                                                                                                                                                                     \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        Task & Method     & $0m$ - $30m$                                & $30m$ - $50m$                                             & $50m-75m$                                                       & $0m$ - $30m$                                & $30m$ - $50m$                               & $50m-75m$                                                       & $0m$ - $30m$                                & $30m$ - $50m$                                                   & $50m-75m$                                                       \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} 
        \multirowcell{6}{KITTI \\ $\downarrow$ \\ Waymo} & SA     & $\phantom{0}5.41$ / $\phantom{0}5.38$       & $\phantom{0}4.05$ / $\phantom{0}3.54$ & $\phantom{0}0.59$ / $\phantom{0}0.42$ & $11.23$ / $10.10$ & $\phantom{0}9.83$ / $\phantom{0}8.39$ & $\phantom{0}1.06$ / $\phantom{0}0.74$ & $16.82$ / $16.70$ & $\phantom{0}6.65$ / $\phantom{0}6.27$ & $\phantom{0}0.35$ / $\phantom{0}0.33$ \\
        \cmidrule(lr){2-11}
             & SN$^\dag$  & $\phantom{0}7.38$ / $\phantom{0}7.19$       & $\phantom{0}0.22$ / $\phantom{0}0.19$                     & $\phantom{0}0.00$ / $\phantom{0}0.00$       & $\phantom{0}4.75$ / $\phantom{0}4.25$       & $\phantom{0}0.07$ / $\phantom{0}0.06$       & $\phantom{0}0.01$ / $\phantom{0}0.01$                           & $\phantom{0}3.81$ / $\phantom{0}3.78$       & $\phantom{0}0.00$ /  $\phantom{0}0.00$      & $\phantom{0}0.00$ /  $\phantom{0}0.00$      \\
             & OT$^\dag$  & $16.48$ / $16.10$                           & $\phantom{0}8.00$ / $\phantom{0}7.00$ & $\phantom{0}1.21$ / $\phantom{0}0.87$                           & $\bestresult{18.18}$ / $\bestresult{16.35}$ & $\bestresult{14.11}$ / $\bestresult{12.05}$ & $\bestresult{\phantom{0}1.48}$ / $\bestresult{\phantom{0}1.03}$ & $\bestresult{24.56}$ / $\bestresult{24.38}$ & $\bestresult{\phantom{0}8.01}$ / $\bestresult{\phantom{0}7.54}$ & $\phantom{0}0.43$ / $\phantom{0}0.40$                           \\
             & ROS$^\dag$ & $\phantom{0}7.31$ / $\phantom{0}7.14$       & $\phantom{0}1.65$ / $\phantom{0}1.44$                     & $\phantom{0}0.08$ / $\phantom{0}0.06$                           & $\phantom{0}7.31$ / $\phantom{0}7.14$       & $\phantom{0}1.65$ / $\phantom{0}1.44$       & $\phantom{0}0.08$ / $\phantom{0}0.06$                           & $\phantom{0}5.29$ / $\phantom{0}5.25$       & $\phantom{0}0.06$ / $\phantom{0}0.05$                           & $\phantom{0}0.00$ /  $\phantom{0}0.00$                          \\
             & TA$^\dag$  & $\bestresult{19.73}$ / $\bestresult{19.28}$ & $\bestresult{10.71}$ / $\bestresult{\phantom{0}9.37}$     & $\phantom{0}1.85$ / $\phantom{0}1.34$                           & $15.45$ / $13.88$                           & $\phantom{0}9.87$ / $\phantom{0}8.41$       & $\phantom{0}0.75$ / $\phantom{0}0.52$                           & $21.39$ / $21.23$                           & $\phantom{0}7.55$ / $\phantom{0}7.11$                           & $\bestresult{\phantom{0}0.46}$ / $\bestresult{\phantom{0}0.43}$ \\
        \cmidrule(lr){2-11}
             & Ours       & $12.12$ / $11.83$                           & $\phantom{0}9.18$ / $\phantom{0}8.04$                     & $\bestresult{\phantom{0}2.02}$ / $\bestresult{\phantom{0}1.46}$ & $11.36$ / $10.22$                           & $10.19$ / $\phantom{0}8.69$                 & $\phantom{0}1.13$ / $\phantom{0}0.79$                           & $16.20$ / $16.08$                           & $\phantom{0}6.37$ / $\phantom{0}6.00$                 & $\phantom{0}0.40$ / $\phantom{0}0.38$                           \\
        \midrule
        \multirowcell{6}{nuScenes \\ $\downarrow$ \\ Waymo} & SA     & $59.56$ / $58.39$ & $15.75$ / $13.82$ & $\phantom{0}2.52$ / $\phantom{0}1.82$ & $\phantom{0}5.24$ / $\phantom{0}4.69$ & $\phantom{0}1.61$ / $\phantom{0}1.37$ & $\phantom{0}0.48$ / $\phantom{0}0.33$ & $\phantom{0}8.68$ / $\phantom{0}8.62$ & $\phantom{0}0.20$ / $\phantom{0}0.19$ & $\bestresult{\phantom{0}0.04}$ / $\bestresult{\phantom{0}0.04}$ \\
        \cmidrule(lr){2-11}
             & SN         & $\bestresult{66.82}$ / $\bestresult{65.52}$                           & $\bestresult{22.93}$ / $\bestresult{20.15}$                                         & $\phantom{0}2.59$ / $\phantom{0}1.87$                           & $\phantom{0}3.74$ / $\phantom{0}3.34$       & $\phantom{0}2.15$ / $\phantom{0}1.82$       & $\phantom{0}0.24$ / $\phantom{0}0.17$                           & $10.11$ / $10.04$                           & $\phantom{0}0.41$ / $\phantom{0}0.38$                           & $\phantom{0}0.01$ / $\phantom{0}0.01$                           \\
             & OT$^\dag$  & $63.51$ / $62.23$                           & $16.80$ / $14.75$                                         & $\phantom{0}2.53$ / $\phantom{0}1.83$                           & $13.63$ / $12.22$                           & $\bestresult{\phantom{0}5.93}$ / $\bestresult{\phantom{0}5.07}$       & $\bestresult{\phantom{0}2.12}$ / $\bestresult{\phantom{0}1.49}$                           & $\phantom{0}4.30$ / $\phantom{0}4.27$       & $\phantom{0}0.12$ / $\phantom{0}0.12$                           & $\phantom{0}0.03$ / $\phantom{0}0.02$                           \\
             & ROS$^\dag$ & $58.56$ / $57.41$                           & $22.05$ / $19.40$                                         & $\bestresult{\phantom{0}5.14}$ / $\bestresult{\phantom{0}3.73}$                           & $\bestresult{16.14}$ / $\bestresult{14.48}$                           & $\phantom{0}1.30$ / $\phantom{0}1.11$       & $\phantom{0}0.19$ / $\phantom{0}0.13$                           & $\bestresult{15.33}$ / $\bestresult{15.22}$                           & $\bestresult{\phantom{0}0.67}$ / $\bestresult{\phantom{0}0.63}$                           & $\phantom{0}0.03$ / $\phantom{0}0.03$                           \\
             & TA$^\dag$  & $62.89$ / $61.63$                           & $17.71$ / $15.55$                                         & $\phantom{0}2.83$ / $\phantom{0}2.05$                           & $11.25$ / $10.09$                           & $\phantom{0}4.33$ / $\phantom{0}3.70$       & $\phantom{0}1.80$ / $\phantom{0}1.27$                           & $\phantom{0}1.77$ / $\phantom{0}1.76$       & $\phantom{0}0.03$ / $\phantom{0}0.03$                                                 & $\phantom{0}0.01$ / $\phantom{0}0.01$                                      \\
        \cmidrule(lr){2-11}
             & Ours       & $60.55$ / $59.32$                           & $14.02$ / $12.30$                                         & $\phantom{0}1.87$ / $\phantom{0}1.35$                           & $\phantom{0}3.83$ / $\phantom{0}3.43$       & $\phantom{0}1.02$ / $\phantom{0}0.87$       & $\phantom{0}0.27$ / $\phantom{0}0.19$                           & $\phantom{0}8.01$ / $\phantom{0}7.95$       & $\phantom{0}0.19$ / $\phantom{0}0.18$                           & $\phantom{0}0.02$ / $\phantom{0}0.02$                           \\
        \bottomrule[1pt]
      \end{tabular}
    }
  \end{center}
  \caption{
    Results of the adaptation from KITTI and nuScenes to Waymo at different distances from the sensor.
    We show $L1$\_AP / $L2$\_AP for the three main classes.
    We compare our method to Source Anchors (SA), Statistical Normalization (SN), Output Transformation (OT), Random Object Scaling (ROS) and Target Anchors (TA).
    % $^\dag$ denotes weakly-supervised methods.
  }
  \label{table:to_waymo_extnsive}
\end{table*}

